Global Scheduling of Weakly-Hard Real-Time Tasks using Job-Level Priority Classes

Real-time systems are intrinsic components of many pivotal applications, such as self-driving vehicles, aerospace and defense systems. The trend in these applications is to incorporate multiple tasks onto fewer, more powerful hardware platforms, e.g., multi-core systems, mainly for reducing cost and power consumption. Many real-time tasks, like control tasks, can tolerate occasional deadline misses due to robust algorithms. These tasks can be modeled using the weakly-hard model. Literature shows that leveraging the weakly-hard model can relax the over-provisioning associated with designed real-time systems. However, a wide-range of the research focuses on single-core platforms. Therefore, we strive to extend the state-of-the-art of scheduling weakly-hard real-time tasks to multi-core platforms. We present a global job-level fixed priority scheduling algorithm together with its schedulability analysis. The scheduling algorithm leverages the tolerable continuous deadline misses to assigning priorities to jobs. The proposed analysis extends the Response Time Analysis (RTA) for global scheduling to test the schedulability of tasks. Hence, our analysis scales with the number of tasks and number of cores because, unlike literature, it depends neither on Integer Linear Programming nor reachability trees. Schedulability analyses show that the schedulability ratio is improved by 40% comparing to the global Rate Monotonic (RM) scheduling and up to 60% more than the global EDF scheduling, which are the state-of-the-art schedulers on the RTEMS real-time operating system. Our evaluation on industrial embedded multi-core platform running RTEMS shows that the scheduling overhead of our proposal does not exceed 60 Nanosecond.

==> bibliography.tex <==
% Encoding: UTF-8

% Richard's anomalies
@article{graham1976bounds,
  title={Bounds on the performance of scheduling algorithms},
  author={Graham, RL},
  journal={Computer and job scheduling theory},
  pages={165--227},
  year={1976},
  publisher={John Wiley and Sons Chichester}
}

@book{buttazzo2011hard,
  title={Hard real-time computing systems: predictable scheduling algorithms and applications},
  author={Buttazzo, Giorgio C},
  volume={24},
  year={2011},
  publisher={Springer Science \& Business Media}
}

% Global multi-processor scheduling worst case behavior problem
@article{baruah2010open,
  title={Open problems in real-time scheduling},
  author={Baruah, Sanjoy and Pruhs, Kirk},
  journal={Journal of Scheduling},
  volume={13},
  number={6},
  pages={577},
  year={2010},
  publisher={Springer Nature BV}
}

% fpEDF
@article{baruah2004optimal,
  title={Optimal utilization bounds for the fixed-priority scheduling of periodic task systems on identical multiprocessors},
  author={Baruah, Sanjoy K},
  journal={IEEE Transactions on Computers},
  volume={53},
  number={6},
  pages={781--784},
  year={2004},
  publisher={IEEE}
}

% EDFk and PriD
@article{goossens2003priority,
  title={Priority-driven scheduling of periodic task systems on multiprocessors},
  author={Goossens, Jo{\"e}l and Funk, Shelby and Baruah, Sanjoy},
  journal={Real-time systems},
  volume={25},
  number={2},
  pages={187--205},
  year={2003},
  publisher={Springer}
}

% RM-US
@inproceedings{andersson2001static,
  title={Static-priority scheduling on multiprocessors},
  author={Andersson, Bj{\"o}rn and Baruah, Sanjoy and Jonsson, Jan},
  booktitle={Proceedings 22nd IEEE Real-Time Systems Symposium (RTSS 2001)(Cat. No. 01PR1420)},
  pages={193--202},
  year={2001},
  organization={IEEE}
}

% DM-DS
@inproceedings{bertogna2005new,
  title={New schedulability tests for real-time task sets scheduled by deadline monotonic on multiprocessors},
  author={Bertogna, Marko and Cirinei, Michele and Lipari, Giuseppe},
  booktitle={International Conference on Principles of Distributed Systems},
  pages={306--321},
  year={2005},
  organization={Springer}
}

@article{bernat2001weakly,
  title={Weakly hard real-time systems},
  author={Bernat, Guillem and Burns, Alan and Liamosi, Albert},
  journal={IEEE transactions on Computers},
  volume={50},
  number={4},
  pages={308--321},
  year={2001},
  publisher={IEEE}
}

@inproceedings{maggio2020control,
  title={Control-system stability under consecutive deadline misses constraints},
  author={Maggio, Martina and Hamann, Arne and Mayer-John, Eckart and Ziegenbein, Dirk},
  booktitle={32nd Euromicro Conference on Real-Time Systems (ECRTS 2020)},
  year={2020},
  organization={Schloss Dagstuhl-Leibniz-Zentrum f{\"u}r Informatik}
}

@InProceedings{vreman2021control,
	author =	{Vreman, Nils and Cervin, Anton and Maggio, Martina},
	title =	{{Stability and Performance Analysis of Control Systems Subject to Bursts of Deadline Misses}},
	booktitle =	{33rd Euromicro Conference on Real-Time Systems (ECRTS 2021)},
	pages =	{15:1--15:23},
	series =	{Leibniz International Proceedings in Informatics (LIPIcs)},
	ISBN =	{978-3-95977-192-4},
	ISSN =	{1868-8969},
	year =	{2021},
	volume =	{196},
	editor =	{Brandenburg, Bj\"{o}rn B.},
	publisher =	{Schloss Dagstuhl -- Leibniz-Zentrum f{\"u}r Informatik},
	address =	{Dagstuhl, Germany},
	URL =		{https://drops.dagstuhl.de/opus/volltexte/2021/13946},
	URN =		{urn:nbn:de:0030-drops-139460},
	doi =		{10.4230/LIPIcs.ECRTS.2021.15},
	annote =	{Keywords: Fault-Tolerant Control Systems, Weakly Hard Task Model}
}

@INPROCEEDINGS{Vreman2022jlWH,
	author={Vreman, Nils and Pates, Richard and Maggio, Martina},
	booktitle={2022 IEEE 28th Real-Time and Embedded Technology and Applications Symposium (RTAS)}, 
	title={WeaklyHard.jl: Scalable Analysis of Weakly-Hard Constraints}, 
	year={2022},
	volume={},
	number={},
	pages={228-240},
	doi={10.1109/RTAS54340.2022.00026}}

@ARTICLE{Vreman2022control,
	author={Vreman, Nils and Pazzaglia, Paolo and Magron, Victor and Wang, Jie and Maggio, Martina},
	journal={IEEE Control Systems Letters}, 
	title={Stability of Linear Systems Under Extended Weakly-Hard Constraints}, 
	year={2022},
	volume={6},
	number={},
	pages={2900-2905},
	doi={10.1109/LCSYS.2022.3179960}}


@article{choi2021toward,
  title={Toward practical weakly hard real-time systems: A job-class-level scheduling approach},
  author={Choi, Hyunjong and Kim, Hyoseung and Zhu, Qi},
  journal={IEEE Internet of Things Journal},
  volume={8},
  number={8},
  pages={6692--6708},
  year={2021},
  publisher={IEEE}
}

@INPROCEEDINGS{choi2019jobclass,
	author={Choi, Hyunjong and Kim, Hyoseung and Zhu, Qi},
	booktitle={2019 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS)}, 
	title={Job-Class-Level Fixed Priority Scheduling of Weakly-Hard Real-Time Systems}, 
	year={2019},
	volume={},
	number={},
	pages={241-253},
	doi={10.1109/RTAS.2019.00028}}

@InProceedings{huang2020safetyWH,
	author={Huang, Chao	and Chang, Kai-Chieh and Lin, Chung-Wei	and Zhu, Qi},
	editor={Lahiri, Shuvendu K. and Wang, Chao},
	title={SAW: A Tool for Safety Analysis of Weakly-Hard Systems},
	booktitle={Computer Aided Verification},
	year={2020},
	publisher={Springer International Publishing},
	address={Cham},
	pages={543--555},
	abstract={We introduce SAW, a tool for safety analysis of weakly-hard systems, in which traditional hard timing constraints are relaxed to allow bounded deadline misses for improving design flexibility and runtime resiliency. Safety verification is a key issue for weakly-hard systems, as it ensures system safety under allowed deadline misses. Previous works are either for linear systems only, or limited to a certain type of nonlinear systems (e.g., systems that satisfy exponential stability and Lipschitz continuity of the system dynamics). In this work, we propose a new technique for infinite-time safety verification of general nonlinear weakly-hard systems. Our approach first discretizes the safe state set into grids and constructs a directed graph, where nodes represent the grids and edges represent the reachability relation. Based on graph theory and dynamic programming, our approach can effectively find the safe initial set (consisting of a set of grids), from which the system can be proven safe under given weakly-hard constraints. Experimental results demonstrate the effectiveness of our approach, when compared with the state-of-the-art. An open source implementation of our tool is available at https://github.com/551100kk/SAW. The virtual machine where the tool is ready to run can be found at https://www.csie.ntu.edu.tw/{\textasciitilde}r08922054/SAW.ova.",
	isbn="978-3-030-53288-8}
}

@inproceedings{huang2019formalWH,
	author = {Huang, Chao and Li, Wenchao and Zhu, Qi},
	title = {Formal Verification of Weakly-Hard Systems},
	year = {2019},
	isbn = {9781450362825},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3302504.3311811},
	doi = {10.1145/3302504.3311811},
	abstract = {Weakly-hard systems are real-time systems that can tolerate occasional deadline misses in a bounded manner. Compared with traditional systems with hard deadline constraints, they provide more scheduling flexibility, and thus expand the design space for system configuration and reconfiguration. A key question for such a system is precisely to what degree it can tolerate deadline misses while still meeting its functional requirements. In this paper, we provide a formal treatment to the verification problem of a general class of weakly-hard systems. We discuss relaxation and over-approximation techniques for managing the complexity of reachability analysis, and develop algorithms based upon these for verifying the safety of weakly-hard systems. Experiments demonstrate the effectiveness of our approach in understanding the impact of and guiding the selection among different weakly-hard constraints.},
	booktitle = {Proceedings of the 22nd ACM International Conference on Hybrid Systems: Computation and Control},
	pages = {197–207},
	numpages = {11},
	keywords = {weakly-hard, safety, formal verification},
	location = {Montreal, Quebec, Canada},
	series = {HSCC '19}
}

@INPROCEEDINGS{liang2020FualtWH,
	author={Liang, Hengyi and Wang, Zhilu and Jiao, Ruochen and Zhu, Qi},
	booktitle={2020 IEEE/ACM International Conference On Computer Aided Design (ICCAD)}, 
	title={Leveraging Weakly-hard Constraints for Improving System Fault Tolerance with Functional and Timing Guarantees}, 
	year={2020},
	volume={},
	number={},
	pages={1-9},
	doi={}
}

@inproceedings{gujarati2013outstanding,
  title={Schedulability analysis of the linux push and pull scheduler with arbitrary processor affinities},
  author={Gujarati, Arpan and Cerqueira, Felipe and Brandenburg, Bj{\"o}rn B},
  booktitle={2013 25th Euromicro Conference on Real-Time Systems},
  pages={69--79},
  year={2013},
  organization={IEEE}
}

@book{baruah2015multiprocessor,
  title={Multiprocessor scheduling for real-time systems},
  author={Baruah, Sanjoy and Bertogna, Marko and Buttazzo, Giorgio},
  year={2015},
  publisher={Springer}
}

% 2 parameter task model / RM
@article{liu1973scheduling,
  title={Scheduling algorithms for multiprogramming in a hard-real-time environment},
  author={Liu, Chung Laung and Layland, James W},
  journal={Journal of the ACM (JACM)},
  volume={20},
  number={1},
  pages={46--61},
  year={1973},
  publisher={ACM New York, NY, USA}
}

% 3 parameter task model / DM
@article{leung1982complexity,
  title={On the complexity of fixed-priority scheduling of periodic, real-time tasks},
  author={Leung, Joseph Y-T and Whitehead, Jennifer},
  journal={Performance evaluation},
  volume={2},
  number={4},
  pages={237--250},
  year={1982},
  publisher={Elsevier}
}

% Optimality impossible
@article{fisher2010optimal,
  title={Optimal online multiprocessor scheduling of sporadic real-time tasks is impossible},
  author={Fisher, Nathan and Goossens, Jo{\"e}l and Baruah, Sanjoy},
  journal={Real-Time Systems},
  volume={45},
  number={1},
  pages={26--71},
  year={2010},
  publisher={Springer}
}

% LET
@incollection{kirsch2012logical,
  title={The logical execution time paradigm},
  author={Kirsch, Christoph M and Sokolova, Ana},
  booktitle={Advances in Real-Time Systems},
  pages={103--120},
  year={2012},
  publisher={Springer}
}

% EDF
@article{horn1974some,
  title={Some simple scheduling algorithms},
  author={Horn, WA},
  journal={Naval Research Logistics Quarterly},
  volume={21},
  number={1},
  pages={177--185},
  year={1974},
  publisher={Wiley Online Library}
}

@inproceedings{wang2002survey,
  title={Survey of weakly-hard real time schedule theory and its application},
  author={Wang, Zhi and Song, Ye-Qiong and Poggi, Enrico-Maria and Sun, Youxian},
  booktitle={International Symposium on Distributed Computing and Applications to Business, Engineering and Science-DCABES'2002},
  pages={9--p},
  year={2002}
}

% DBP / streams (m,k)
@article{hamdaoui1995dynamic,
  title={A dynamic priority assignment technique for streams with (m, k)-firm deadlines},
  author={Hamdaoui, Moncef and Ramanathan, Parameswaran},
  journal={IEEE transactions on Computers},
  volume={44},
  number={12},
  pages={1443--1451},
  year={1995},
  publisher={IEEE}
}

% DWC
@inproceedings{lehoczky1989rate,
  title={The rate monotonic scheduling algorithm: Exact characterization and average case behavior},
  author={Lehoczky, John and Sha, Lui and Ding, Yuqin},
  booktitle={RTSS},
  volume={89},
  pages={166--171},
  year={1989}
}

% ERM
@article{hamsaoui1997evaluating,
  title={Evaluating dynamic failure probability for streams with (m, k)-firm deadlines},
  author={Hamsaoui, M and Ramanathan, Parameswaran},
  journal={IEEE Transactions on Computers},
  volume={46},
  number={12},
  pages={1325--1337},
  year={1997},
  publisher={IEEE}
}

% D-over
@phdthesis{koren1992d,
  title={D-OVER; an optimal on-line scheduling algorithm for overloaded real-time systems},
  author={Koren, Gilad and Shasha, Dennis},
  year={1992},
  school={Inria}
}

% RTO BWP
@inproceedings{koren1995skip,
  title={Skip-over: Algorithms and complexity for overloaded systems that allow skips},
  author={Koren, Gilad and Shasha, Dennis},
  booktitle={Proceedings 16th IEEE Real-Time Systems Symposium},
  pages={110--117},
  year={1995},
  organization={IEEE}
}

% EDL-RTO EDL-BWP
@article{marchand2006dynamic,
  title={Dynamic real-time scheduling of firm periodic tasks with hard and soft aperiodic tasks},
  author={Marchand, Audrey and Silly-Chetto, Maryline},
  journal={Real-Time Systems},
  volume={32},
  number={1},
  pages={21--47},
  year={2006},
  publisher={Springer}
}

% RLP
@inproceedings{chetto2007dynamic,
  title={Dynamic scheduling of skippable periodic tasks in weakly-hard real-time systems},
  author={Chetto, Maryline and Marchand, Audrey},
  booktitle={14th Annual IEEE International Conference and Workshops on the Engineering of Computer-Based Systems (ECBS'07)},
  pages={171--177},
  year={2007},
  organization={IEEE}
}

% RLP/T
@inproceedings{marchand2008dynamic,
  title={Dynamic scheduling of periodic skippable tasks in an overloaded real-time system},
  author={Marchand, Audrey and Chetto, Maryline},
  booktitle={2008 IEEE/ACS International Conference on Computer Systems and Applications},
  pages={456--464},
  year={2008},
  organization={IEEE}
}

% CBS
@inproceedings{abeni1998integrating,
  title={Integrating multimedia applications in hard real-time systems},
  author={Abeni, Luca and Buttazzo, Giorgio},
  booktitle={Proceedings 19th IEEE Real-Time Systems Symposium (Cat. No. 98CB36279)},
  pages={4--13},
  year={1998},
  organization={IEEE}
}

% CBS
@article{abeni2004resource,
  title={Resource reservation in dynamic real-time systems},
  author={Abeni, Luca and Buttazzo, Giorgio},
  journal={Real-Time Systems},
  volume={27},
  number={2},
  pages={123--167},
  year={2004},
  publisher={Springer}
}

% CASH
@article{caccamo2005efficient,
  title={Efficient reclaiming in reservation-based real-time systems with variable execution times},
  author={Caccamo, Marco and Buttazzo, Giorgio C and Thomas, Deepu C},
  journal={IEEE Transactions on Computers},
  volume={54},
  number={2},
  pages={198--213},
  year={2005},
  publisher={IEEE}
}

% IRIS
@inproceedings{marzario2004iris,
  title={Iris: A new reclaiming algorithm for server-based real-time systems},
  author={Marzario, Luca and Lipari, Giuseppe and Balbastre, Patricia and Crespo, Alfons},
  booktitle={Proceedings. RTAS 2004. 10th IEEE Real-Time and Embedded Technology and Applications Symposium, 2004.},
  pages={211--218},
  year={2004},
  organization={IEEE}
}

% BACKSLASH
@inproceedings{lin2005improving,
  title={Improving soft real-time performance through better slack reclaiming},
  author={Lin, Caixue and Brandt, Scott A},
  booktitle={26th IEEE International Real-Time Systems Symposium (RTSS'05)},
  pages={12--pp},
  year={2005},
  organization={IEEE}
}

% BWI
@inproceedings{lamastra2001bandwidth,
  title={A bandwidth inheritance algorithm for real-time task synchronization in open systems},
  author={Lamastra, Gerardo and Lipari, Giuseppe and Abeni, Luca},
  booktitle={Proceedings 22nd IEEE Real-Time Systems Symposium (RTSS 2001)(Cat. No. 01PR1420)},
  pages={151--160},
  year={2001},
  organization={IEEE}
}

% SIRAP
@inproceedings{behnam2007sirap,
  title={Sirap: a synchronization protocol for hierarchical resource sharingin real-time open systems},
  author={Behnam, Moris and Shin, Insik and Nolte, Thomas and Nolin, Mikael},
  booktitle={Proceedings of the 7th ACM \& IEEE international conference on Embedded software},
  pages={279--288},
  year={2007}
}

% SIRAP
@article{nolte2009synchronization,
  title={A synchronization protocol for temporal isolation of software components in vehicular systems},
  author={Nolte, Thomas and Shin, Insik and Behnam, Moris and Sjodin, Mikael},
  journal={IEEE Transactions on Industrial Informatics},
  volume={5},
  number={4},
  pages={375--387},
  year={2009},
  publisher={IEEE}
}

@inproceedings{davis2006resource,
  title={Resource sharing in hierarchical fixed priority pre-emptive systems},
  author={Davis, Robert I and Burns, Alan},
  booktitle={2006 27th IEEE International Real-Time Systems Symposium (RTSS'06)},
  pages={257--270},
  year={2006},
  organization={IEEE}
}

@inproceedings{behnam2008scheduling,
  title={Scheduling of semi-independent real-time components: Overrun methods and resource holding times.},
  author={Behnam, Moris and Shin, Insik and Nolte, Thomas and Nolin, Mikael},
  booktitle={2008 IEEE International Conference on Emerging Technologies and Factory Automation},
  pages={575--582},
  year={2008},
  organization={IEEE}
}

@article{behnam2009overrun,
  title={Overrun methods and resource holding times for hierarchical scheduling of semi-independent real-time systems},
  author={Behnam, Moris and Nolte, Thomas and Sjodin, Mikael and Shin, Insik},
  journal={IEEE Transactions on Industrial Informatics},
  volume={6},
  number={1},
  pages={93--104},
  year={2009},
  publisher={IEEE}
}

@inproceedings{lin1987concord,
  title={Concord: A system of imprecise computation},
  author={Lin, K-J},
  booktitle={Proceedings of the Eleventh Annual International Computer Software and Applications Conference (COMPSAC 87)},
  year={1987}
}

@techreport{liu1987scheduling,
  title={Scheduling real-time, periodic jobs using imprecise results},
  author={Liu, Jane WS and Lin, Kwei-Jay and Natarajan, Swaminathan},
  year={1987}
}

@incollection{liu1991algorithms,
  title={Algorithms for scheduling imprecise computations},
  author={Liu, Jane W.-S. and Lin, Kwei-Jay and Shih, Wei Kuan and Yu, Albert Chuang-shi and Chung, Jen-Yao and Zhao, Wei},
  booktitle={Foundations of Real-Time Computing: Scheduling and Resource Management},
  pages={203--249},
  year={1991},
  publisher={Springer}
}

@article{shih1991algorithms,
  title={Algorithms for scheduling imprecise computations with timing constraints},
  author={Shih, Wei-Kuan and Liu, Jane WS and Chung, Jen-Yao},
  journal={SIAM Journal on Computing},
  volume={20},
  number={3},
  pages={537--552},
  year={1991},
  publisher={SIAM}
}

@article{liu1994imprecise,
  title={Imprecise computations},
  author={Liu, Jane WS and Shih, Wei-Kuan and Lin, Kwei-Jay and Bettati, Riccardo and Chung, Jen-Yao},
  journal={Proceedings of the IEEE},
  volume={82},
  number={1},
  pages={83--94},
  year={1994},
  publisher={IEEE}
}

@book{natarajan1995imprecise,
  title={Imprecise and Approximate Computation},
  author={Natarajan, Swaminathan},
  volume={318},
  year={1995},
  publisher={Springer Science \& Business Media}
}

% Elastic model
@inproceedings{buttazzo1998elastic,
  title={Elastic task model for adaptive rate control},
  author={Buttazzo, Giorgio C and Lipari, Giuseppe and Abeni, Luca},
  booktitle={Proceedings 19th IEEE Real-Time Systems Symposium (Cat. No. 98CB36279)},
  pages={286--295},
  year={1998},
  organization={IEEE}
}

% Elastic model extended
@article{buttazzo2002elastic,
  title={Elastic scheduling for flexible workload management},
  author={Buttazzo, Giorgio C and Lipari, Giuseppe and Caccamo, Marco and Abeni, Luca},
  journal={IEEE Transactions on Computers},
  volume={51},
  number={3},
  pages={289--302},
  year={2002},
  publisher={IEEE}
}

% RED
@book{buttazzo1993red,
  title={RED: Robust earliest deadline scheduling},
  author={Buttazzo, Giorgio C and Stankovic, John A},
  year={1993},
  publisher={University of Massachusetts, Department of Computer Science}
}

% RED
@incollection{buttazzo1995adding,
  title={Adding robustness in dynamic preemptive scheduling},
  author={Buttazzo, Giorgio C and Stankovic, John A},
  booktitle={Responsive Computer Systems: Steps Toward Fault-Tolerant Real-Time Systems},
  pages={67--88},
  year={1995},
  publisher={Springer}
}

% Control signal
@inproceedings{linsenmayer2017stabilization,
  title={Stabilization of networked control systems with weakly hard real-time dropout description},
  author={Linsenmayer, Steffen and Allgower, Frank},
  booktitle={2017 IEEE 56th Annual Conference on Decision and Control (CDC)},
  pages={4765--4770},
  year={2017},
  organization={IEEE}
}

% System level action
@inproceedings{pazzaglia2019dmac,
  title={DMAC: Deadline-miss-aware control},
  author={Pazzaglia, Paolo and Mandrioli, Claudio and Maggio, Martina and Cervin, Anton},
  booktitle={31st Euromicro Conference on Real-Time Systems (ECRTS 2019)},
  year={2019},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}
%TWCA:DATE2012
@inproceedings{quinton2012TWCA,
	author = {Quinton, Sophie and Hanke, Matthias and Ernst, Rolf},
	title = {Formal Analysis of Sporadic Overload in Real-Time Systems},
	year = {2012},
	isbn = {9783981080186},
	publisher = {EDA Consortium},
	address = {San Jose, CA, USA},
	booktitle = {Proceedings of the Conference on Design, Automation and Test in Europe},
	pages = {515–520},
	numpages = {6},
	location = {Dresden, Germany},
	series = {DATE '12}
}
%TWCA:EMSOFT2014
@INPROCEEDINGS{hammadeh2014TWCA,
	author={H. Hammadeh, Zain A. and Quinton, Sophie and Ernst, Rolf},  
	booktitle={2014 International Conference on Embedded Software (EMSOFT)},   
	title={Extending typical worst-case analysis using response-time dependencies to bound deadline misses},   
	year={2014},  
	volume={},  
	number={},  
	pages={1-10},  
	doi={10.1145/2656045.2656059}}

%TWCA:ECRTS2015
@INPROCEEDINGS{xu2015TWCA,
	author={Xu, Wenbo and H. Hammadeh, Zain A. and Kr\"{o}ller, Alexander and Ernst, Rolf and Quinton, Sophie},
	booktitle={2015 27th Euromicro Conference on Real-Time Systems}, 
	title={Improved Deadline Miss Models for Real-Time Systems Using Typical Worst-Case Analysis}, 
	year={2015},
	volume={},
	number={},
	pages={247-256},
	doi={10.1109/ECRTS.2015.29}}

%TWCA:DATE2017
@INPROCEEDINGS{hammadeh2017TWCA,  
	author={H. Hammadeh, Zain A. and Ernst, Rolf and Quinton, Sophie and Henia, Rafik and Rioux, Laurent},  
	booktitle={Design, Automation \& Test in Europe Conference \& Exhibition (DATE), 2017},   
	title={Bounding deadline misses in weakly-hard real-time systems with task dependencies},   
	year={2017},  
	volume={},  
	number={},  
	pages={584-589},  
	doi={10.23919/DATE.2017.7927054}}

%TWCA:ETFA2018
@INPROCEEDINGS{hammadeh2018TWCA,
	author={H. Hammadeh, Zain A. and Ernst, Rolf},  
	booktitle={2018 IEEE 23rd International Conference on Emerging Technologies and Factory Automation (ETFA)},   
	title={Weakly-Hard Real-Time Guarantees for Weighted Round-Robin Scheduling of Real-Time Messages},   
	year={2018},  
	volume={1},  
	number={},  
	pages={384-391},  
	doi={10.1109/ETFA.2018.8502621}}

%TWCA:TECS2019
@article{hammadeh2019TWCA,
	author = {H. Hammadeh, Zain A.  and Quinton, Sophie and Ernst, Rolf},
	title = {Weakly-Hard Real-Time Guarantees for Earliest Deadline First Scheduling of Independent Tasks},
	year = {2019},
	issue_date = {November 2019},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	volume = {18},
	number = {6},
	issn = {1539-9087},
	url = {https://doi.org/10.1145/3356865},
	doi = {10.1145/3356865},
	journal = {ACM Trans. Embed. Comput. Syst.},
	month = {dec},
	articleno = {121},
	numpages = {25},
	keywords = {Weakly hard real-time systems, dynamic priority scheduling, schedulability analysis}}

%MILP
@article{sun2017MILP,
	author = {Sun, Youcheng and Natale, Marco Di},
	title = {Weakly Hard Schedulability Analysis for Fixed Priority Scheduling of Periodic Real-Time Tasks},
	year = {2017},
	issue_date = {October 2017},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	volume = {16},
	number = {5s},
	issn = {1539-9087},
	url = {https://doi.org/10.1145/3126497},
	doi = {10.1145/3126497},
	journal = {ACM Trans. Embed. Comput. Syst.},
	month = {sep},
	articleno = {171},
	numpages = {19},
	keywords = {Weakly hard real-time systems, resource sharing, periodic real-time tasks, activation jitter, schedulability analysis}}

%RTA
@INPROCEEDINGS{bertogna2007response,
	author={Bertogna, Marko and Cirinei, Michele},
	booktitle={28th IEEE International Real-Time Systems Symposium (RTSS 2007)}, 
	title={Response-Time Analysis for Globally Scheduled Symmetric Multiprocessor Platforms}, 
	year={2007},
	volume={},
	number={},
	pages={149-160},
	doi={10.1109/RTSS.2007.31}}

%ODARIS
@inproceedings{schwenk2020ODARIS,
	year = {2020},
	author = {Kurt Schwenk and Daniel Herschmann},
	month = {October},
	title = {On-Board Data Analysis and Real-Time Information System},
	booktitle = {Deutscher Luft- und Raumfahrtkongress 2020},
	abstract = {The DLR is currently working on an on-board data analysis and real-time information system, for satellites and other autonomous platforms. The system should offer query and alarming services with a query-response time of a few minutes. This is hard to archive today and would beneficial for many earth observation applications. A first prototype of the system has been designed and tested on a flight campaign. In this article we present the current status of the system, the next development steps for bringing the system closer to space, and the obstacles we have to tackle on the way.},
	url = {https://elib.dlr.de/137250/},
	keywords = {onboard data analysis, onboard realtime services}
}

%MMX
@inproceedings{barthelmes2022MMX,
	year = {2022},
	month = {March},
	author = {Stefan Barthelmes and Thomas Bahls and Ralph Bayer and Wieland Bertleff and Markus Bihler and Fabian Buse and Maxime Chalon and Franz Hacker and Roman Holderried and Viktor Langofer and Roy Lichtenheldt and Sascha Oliver Moser and Kaname Sasaki and Hans-J{\"u}rgen Sedlmayr and Juliane Skibbe and Leon Stubbig and Bernhard Vodermayer},
	publisher = {IEEE},
	booktitle = {IEEE Aerospace Conference},
	title = {MMX Rover Locomotion Subsystem - Development and
	Testing towards the Flight Model},
	journal = {2022 IEEE Aerospace Conference, AERO 2022},
	keywords = {Space Exploration; Robotics; Locomotion; Chassis; Mechatronics; Rover},
	abstract = {Wheeled rovers have been successfully used as mobile landers on Mars and Moon and more such missions are in the planning. For the Martian Moon eXploration (MMX) mission of the Japan Aerospace Exploration Agency (JAXA), such a wheeled rover will be used on the Marsian Moon Phobos. This is the first rover that will be used under such low gravity, called milli-g, which imposes many challenges to the design of the locomotion subsystem (LSS). The LSS is used for unfolding, standing up, driving, aligning and lowering the rover on Phobos. It is a entirely new developed highly-integrated mechatronic system that is specifically designed for Phobos.
	Since the Phase A concept of the LSS, which was presented two years ago [1], a lot of testing, optimization and design improvements have been done. Following the tight mission schedule, the LSS qualification and flight models (QM and FM) assembly has started in Summer 2021. In this work, the final FM design is presented together with selected test and optimization results that led to the final state. More specifically, advances in the mechanics, electronics, thermal, sensor, firmware and software design are presented.
	The LSS QM and FM will undergo a comprehensive qualification and acceptance testing campaign, respectively, in the first half of 2022 before the FM will be integrated into the rover},
	url = {https://elib.dlr.de/186923/}
}

% UUnifast
@article{bini2005measuring,
  title={Measuring the performance of schedulability tests},
  author={Bini, Enrico and Buttazzo, Giorgio C},
  journal={Real-Time Systems},
  volume={30},
  number={1},
  pages={129--154},
  year={2005},
  publisher={Springer}
}

@article{Baruah2005ProportionatePA,
	title={Proportionate progress: A notion of fairness in resource allocation},
	author={Sanjoy K. Baruah and N. K. Cohen and C. Greg Plaxton and Donald A. Varvel},
	journal={Algorithmica},
	year={2005},
	volume={15},
	pages={600-625}
}

@INPROCEEDINGS{Anderson-Pfair-2000,	
	author={J. H. {Anderson} and A. {Srinivasan}},	
	booktitle={Proceedings Seventh International Conference on Real-Time Computing Systems and Applications}, 	
	title={{Pfair} scheduling: beyond periodic task systems}, 
	year={2000},	
	volume={},	
	number={},	
	pages={297-306},}

@INPROCEEDINGS{Nelissen-UEDF2012,
	author={G. {Nelissen} and V. {Berten} and V. {Nélis} and J. {Goossens} and D. {Milojevic}},
	booktitle={2012 24th Euromicro Conference on Real-Time Systems}, 
	title={U-EDF: An Unfair But Optimal Multiprocessor Scheduling Algorithm for Sporadic Tasks}, 
	year={2012},
	volume={},
	number={},
	pages={13-23},}

@INPROCEEDINGS{Andersson2001,
	author={B. {Andersson} and S. {Baruah} and J. {Jonsson}},
	booktitle={Proceedings 22nd IEEE Real-Time Systems Symposium (RTSS 2001) (Cat. No.01PR1420)}, 
	title={Static-priority scheduling on multiprocessors}, 
	year={2001},
	volume={},
	number={},
	pages={193-202},}

@Inproceedings{Pazzaglia:ECRTS2018,
	author =	{Paolo Pazzaglia and Luigi Pannocchi and Alessandro Biondi and Marco Di Natale},
	title =	{{Beyond the Weakly Hard Model: Measuring the Performance Cost of Deadline Misses}},
	booktitle =	{30th Euromicro Conference on Real-Time Systems (ECRTS 2018)},
	pages =	{10:1--10:22},
	lnseries =	{Leibniz International Proceedings in Informatics (LIPIcs)},
	ISBN =	{978-3-95977-075-0},
	ISSN =	{1868-8969},
	year =	{2018},
	volume =	{106},
	lnpublisher =	{Schloss Dagstuhl--Leibniz-Zentrum fuer Informatik},
	lnaddress =	{Dagstuhl, Germany},
	URL =		{http://drops.dagstuhl.de/opus/volltexte/2018/8993},
	URN =		{urn:nbn:de:0030-drops-89930},
	doi =		{10.4230/LIPIcs.ECRTS.2018.10},
	annote =	{Keywords: control, real-time, cyber physical systems, weakly hard, deadline miss, performance}
}

@Inproceedings{Hammadeh2017ECRTS,
	ADDRESS = "Dubrovnik, Croatia",
	AUTHOR = "Zain A. H. Hammadeh and et al.",
	longAUTHOR = "Zain A. H. Hammadeh and Sophie Quinton and Marco Panunzio and Rafik Henia and Laurent Rioux and Rolf Ernst",
	BOOKTITLE = "The 29th Euromicro Conference on Real-Time Systems (ECRTS17)",
	MONTH = "June",
	TITLE = "Budgeting Under-specified Tasks for Weakly-Hard Real-Time Systems",
	URL = "https://drops.dagstuhl.de/opus/volltexte/2017/7163/",
	YEAR = "2017",
}

@INPROCEEDINGS{Wu2008,
	author={ {Tong Wu} and {Shiyao Jin}},
	booktitle={2008 First IEEE International Conference on Ubi-Media Computing},
	title={Weakly hard real-time scheduling algorithm for multimedia embedded system on multiprocessor platform},
	year={2008},
	volume={},
	number={},
	pages={320-325},
	keywords={media streaming;multimedia systems;multiprocessing systems;quality of service;real-time scheduling algorithm;multimedia embedded system;multiprocessor architectures;embedded systems;multimedia embedded systems;QoS guarantee;real-time tasks;resource constraint;optimistic algorithm;Real time systems;Scheduling algorithm;Multimedia systems;Embedded system;Streaming media;Processor scheduling;Job shop scheduling;Very large scale integration;Computer architecture;Laboratories;Multimedia Stream;Multiprocessor;Weakly Hard Real-Time;Resource Constraint;Integrated Schedule},
	doi={10.1109/UMEDIA.2008.4570910},
	ISSN={null},
	month={July},
}

@INPROCEEDINGS{Kong2011,
	author={Y. {Kong} and H. {Cho}}, 
	booktitle={2011 12th International Conference on Parallel and Distributed Computing, Applications and Technologies}, 
	title={Guaranteed Scheduling for (m,k)-firm Deadline-Constrained Real-Time Tasks on Multiprocessors}, 
	year={2011}, 
	volume={}, 
	number={}, 
	pages={18-23},
} 

 @inproceedings{Quinton12TWCA,
	author    = {Sophie Quinton and
	Matthias Hanke and
	Rolf Ernst},
	title     = {Formal analysis of sporadic overload in real-time systems},
	booktitle = {Proceedings of DATE'12},
	year      = {2012},
	pages     = {515-520},
	ee        = {http://ieeexplore.ieee.org/xpl/freeabs_all.jsp?arnumber=6176523},
	publisher = {IEEE},
	bibsource = {DBLP, http://dblp.uni-trier.de}
}

% Callisto

% HNS
@inproceedings{schwarz2019preliminary,
  title={Preliminary Design of the Hybrid Navigation System (HNS) for the CALLISTO RLV Demonstrator},
  author={Schwarz, Ren{\'e} and Solari, Marco and Razgus, Bronislovas and Dumke, Michael and Markgraf, Markus and Bestard K{\"o}rner, Matias and Pfau, Dennis and Reigenborn, Martin and Braun, Benjamin and Sommer, Jan},
  booktitle={8th European Conference for Aeronautics and Space Sciences (EUCASS)},
  year={2019}
}

@inproceedings{krummen2021towards,
  title={Towards a reusable first stage demonstrator: Callisto-technical progresses \& challenges},
  author={Krummen, Sven and Desmariaux, Jean and Saito, Yasuhiro and Boldt, Marcelo and Briese, Lale Evrim and Cesco, Nathalie and Chavagnac, Christophe and CLIQUET-MORENO, Elisa and Dumont, Etienne and Ecker, Tobias and others},
  booktitle={Proceedings of the International Astronautical Congress, IAC},
  year={2021}
}

@inproceedings{illig2022callisto,
           month = {Juni},
          author = {Illig, Michel and Ishimoto, Shinji and Dumont, Etienne},
           title = {{CALLISTO}, a demonstrator for reusable launchers},
            year = {2022},
       booktitle = {9th European Conference for Aeronautics and Space Sciences (EUCASS)}
}

@Article{app131810131,
AUTHOR = {Han, Sangchul and Paik, Woojin and Ko, Myeong-Cheol and Park, Minkyu},
TITLE = {A Comparative Study on the Schedulability of the EDZL Scheduling Algorithm on Multiprocessors},
JOURNAL = {Applied Sciences},
VOLUME = {13},
YEAR = {2023},
NUMBER = {18},
ARTICLE-NUMBER = {10131},
URL = {https://www.mdpi.com/2076-3417/13/18/10131},
ISSN = {2076-3417},
ABSTRACT = {As multiprocessor (or multicore) real-time systems become popular, there has been much research on multiprocessor real-time scheduling algorithms. This work evaluates EDZL (Earliest Deadline until Zero Laxity), a scheduling algorithm for real-time multiprocessor systems. First, we compare the performance of EDZL schedulability tests. We measure and compare the ratio of task sets admitted by each test. We also investigate the dominance between EDZL schedulability tests and discover that the union of the demand-based test and the utilization-based test is an effective combination. Second, we compare the schedulability of EDZL and EDF(k). We prove that the union of the EDZL schedulability tests dominates the EDF(k) schedulability test, i.e., the union of the EDZL schedulability tests can admit all task sets admitted by the EDF(k) schedulability test. We also compare the schedulability of EDZL and EDF(k) through scheduling simulation by measuring the ratio of successfully scheduled task sets. EDZL can successfully schedule 7.0% more task sets than EDF(k).},
DOI = {10.3390/app131810131}
}

@inproceedings{hammadeh2017budgeting,
  title={Budgeting under-specified tasks for weakly-hard real-time systems},
  author={Hammadeh, Zain AH and Quinton, Sophie and Panunzio, Marco and Henia, Rafik and Rioux, Laurent and Ernst, Rolf},
  booktitle={29th Euromicro Conference on Real-Time Systems (ECRTS 2017)},
  year={2017},
  organization={Schloss-Dagstuhl-Leibniz Zentrum f{\"u}r Informatik}
}

@misc{Natale-ESWEEK17,
	author = "Marco Di Natale",
	title = "Beyond the m-k model: restoring performance considerations in the time abstraction",
	year = "2017",
	note   = "ESWEEK - Tutorial Slides",
	booktitle={EMBEDDED SYSTEM WEEK},
	location = {Seoul, South Korea},
}
